Catapults in SGD: spikes in the training loss and their impact on generalization through feature learning

In this paper, we first present an explanation regarding the common occurrence of spikes in the training loss when neural networks are trained with stochastic gradient descent (SGD). We provide evidence that the spikes in the training loss of SGD are "catapults", an optimization phenomenon originally observed in GD with large learning rates in [Lewkowycz et al. 2020]. We empirically show that these catapults occur in a low-dimensional subspace spanned by the top eigenvectors of the tangent kernel, for both GD and SGD. Second, we posit an explanation for how catapults lead to better generalization by demonstrating that catapults promote feature learning by increasing alignment with the Average Gradient Outer Product (AGOP) of the true predictor. Furthermore, we demonstrate that a smaller batch size in SGD induces a larger number of catapults, thereby improving AGOP alignment and test performance.

==> arxiv_do_not_read_this__/catapult_dynamics_linearity.tex <==
\section{Catapult dynamics and linear training regime}
In this section, we empirically show that models that can have linear training regime with MSE trained with GD  will exhibit catapult dynamics. We start with the linear training regime, which is closely related to the property of transition to linearity, or the constancy of NTK.

\subsection{Linear training regime}
Consider the following $L$-layer fully-connected neural network given input $\vx\in\mathbb{R}^d$:
\begin{align}\label{eq:generalnn}
 &f^{(0)} = \vx, \nonumber\\
 &f^{(\ell)}= \sigma\left(\alpha_{\ell-1}W^{(\ell)}f^{(\ell-1)}\right), \ \forall l = 1,2,\cdots, L-1,\nonumber\\
 &f = f^{(L)} = \alpha_{L-1}\rvv^T f^{(L-1)},
\end{align}
where $W^{(\ell)}\in\mathbb{R}^{m_{\ell}\times m_{\ell-1}}$ for $\ell\in[L-1]$, $\rvv\in\mathbb{R}^{m_{L-1}}$ are trainable weight parameters, $\sigma(\cdot)$ is an element-wise activation function, and $\alpha_\ell \in \mathbb{R}$ is the scaling factor which possibly depends on $m_{\ell-1}$. We assume all the hidden layers have the same width $m$, i.e., $m_{\ell} = m$ for $\ell\in[L-1]$.

We denote $\tW:=(W^{(1)},\cdots,W^{(L-1)},\rvv:=W^{(L)})$ as the collection of all trainable parameters, hence the network function can be written as  $f(\tW;\vx)$.

\paragraph{Network parameterization.} Each trainable weight parameter in $W^{(\ell)}$ is i.i.d. drawn from $\mathcal{N}(0,\kappa_\ell^2)$ for $\ell\in[L]$. The variance is chosen $\kappa_\ell = \frac{1}{\alpha_\ell\sqrt{m}}$ for $\ell \in [L-1]$ and $\kappa_0 = \frac{1}{\alpha_0\sqrt{d}}$.

\begin{remark}
Under network parameterization, each neuron is of the order of $\tilde{O}(1)$ with respect to $m$ with high probability over random initialization.
\end{remark}

\begin{remark}
When $\kappa_\ell= 1$ for all $\ell$, the above parameterization is exactly NTK parameterization.  When $\kappa_\ell = 1/\sqrt{m}$ for $\ell\in[L]$ and $\kappa_0 = 1/\sqrt{d}$, the above parameterization is standard initialization or so-called Lecun's initialization.
\end{remark}




\begin{thm}[Transition to linearity]
Given network $f(\tW)$, under network parameterization, with high probability over random initialization of $\tW_0$, in the ball $B(\tW_0, R)$ with $R = O(\min_\ell \kappa_\ell)$,
\begin{align*}
    \frac{\|H_f\|}{\|K_f\|} = \tilde{O}(1/\sqrt{m}).
\end{align*}
\end{thm}

\begin{corollary}[Linear training regime]

\end{corollary}




The above results can be extended to CNNs, ResNets, or the mixture of those layers~\cite{liu2020loss}.


\subsection{Sufficient condition for catapult dynamics}
Now we state our empirical observation: with appropriately chosen learning rates,
\begin{center}
    \textit{\textbf{Transition to linearity + MSE + GD 
    $\Longrightarrow$ Catapult dynamics.}}
\end{center}

More precisely, for neural networks which have the property of transition to linearity, if we train such models with MSE by gradient descent, we can observe catapult dynamics when the learning rate is chosen appropriately large. We empirically observe that in this setting, it suffices to choose a learning rate larger than $\frac{2n}{\lambda_{\max} (K(\rvw_0))}$ to produce catapult dynamics if the network is wide.

In the following, we enumerate the empirical observations in catapult dynamics. 

\paragraph{Effects of the learning rate and the width.}
In the catapult dynamics, two major metrics we are concerned with are the height of the loss spikes and the size of $\lambda_{\max}(K)$ at convergence. We typically observe that 1) a larger learning rate leads to a higher spike and a smaller $\lambda_{\max}(K)$ at convergence; 2)a larger width also leads to a higher spike but comparable size of $\lambda_{\max}(K)$ at convergence. Similar phenomena were observed in~\cite{lewkowycz2020large,zhu2022quadratic} as well.

% \begin{figure}[h]
%      \centering
%      \begin{subfigure}[b]{0.48\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figure/loss_gd.png}
%          \caption{NTK parameterization}
%          \label{fig:y equals x}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.48\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figure/ntk_gd.png}
%          \caption{NTK parameterization}
%          \label{fig:three sin x}
%      \end{subfigure}
% \end{figure}








==> arxiv_do_not_read_this__/catapult_general.tex <==

\section{Catapult dynamics in more general settings}
We have shown that with gradient descent, we can consistently observe catapult dynamics. In this section, we will demonstrate that catapult dynamics can be observed with other gradient-based algorithms, e.g., SGD, Adam, Adagrad, and Adadelta, and with momentum. We observe that the training phenomenon in such general settings is not exactly the same as the one training with GD. The loss may not exhibit clear spikes but mild oscillations. However, we can consistently see that $\lambda_{\max}(K)$ decreases and it decreases more when the learning rate gets larger.

The loss does not necessarily have spikes but top eigenvalues of NTK decrease.
It can be generalized to 
\begin{center}
    \textit{\textbf{Transition to linearity + MSE + Gradient-based algorithm 
    $\Longrightarrow$ Catapult dynamics.}}
\end{center}

\begin{figure}[h]
     \centering
    \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/loss_resnet_mom.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/ntk_resnet_mom.png}
     \end{subfigure}
     \caption{Momentum}
\end{figure}

\begin{figure}[h]
     \centering
    \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/loss_resnet_adam.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/ntk_resnet_adam.png}
     \end{subfigure}
     \caption{Adam}
\end{figure}

\begin{figure}[h]
     \centering
    \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/loss_resnet_adagrad.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/ntk_resnet_adagrad.png}
     \end{subfigure}
     \caption{Adagrad}
\end{figure}

==> arxiv_do_not_read_this__/other_losses.tex <==
\section{Other losses and parameterization}

With losses other than square loss, or with parameterization other than NTK parameterization, the GD typically does not have a critical learning rate, hence there is no consistent catapult dynamics.

\paragraph{Example: mean field parameterization}

\begin{figure}[htb!]
     \centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/loss_cnn_mf.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/ntk_cnn_mf.png}
     \end{subfigure}
             \caption{Mean field parameterization}
\end{figure}

\paragraph{Example: cross-entropy loss}
\begin{figure}[htb!]
     \centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/loss_cnn_logi.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/ntk_cnn_logi.png}
     \end{subfigure}
              \caption{Logistic loss}
\end{figure}
